VIB is Half Bayes

In discriminative settings such as regression and classification there are two random variables at play, the inputs X and the targets Y. Here, we demonstrate that the Variational Information Bottleneck can be viewed as a compromise between fully empirical and fully Bayesian objectives, attempting to minimize the risks due to finite sampling of Y only. We argue that this approach provides some of the benefits of Bayes while requiring only some of the work.

==> tex/oldBayesPAC.tex <==

\section{Bayes and MLE}
\fixme{Honestly should probably cut this whole section}
Why does Bayesian inference generate better predictions than Maximum Likelihood?
Bayesian inference and Maximum likelihood agree 
asymptotically.
Bayesian inference however is able to provide 
guarantees in the limit of finite data that 
Maximum Likelihood cannot.  Both camps aim to
minimize the \emph{inferential risk}:
\begin{equation}
    \label{eqn:trueinfrisk}
    \mathcal R[q] \equiv \mathbb{E}_{q(\Theta)} [ L(\theta)] \qquad L(\theta) \equiv -\mathbb{E}_{\nu(X)}[ \log p(X|\Theta) ],
\end{equation}
seeking a distribution in parameter space ($q(\Theta)$) 
which achieves the best average log likelihood ($\log p(X|\Theta)$) over the \emph{true} data distribution ($\nu(X)$), or lowest \emph{true loss} $L(\theta)$. 
The optimal parameter distribution will be 
an atomic distribution $q^*(\Theta) = \argmin_{q(\Theta)} \mathcal R = \delta(\Theta - \Theta_0)$ on the best single setting of the parameters of the model $p(X|\Theta)$.  This could be viewed as 
performing variational optimization~\citep{varopt} for the parameter setting $\theta$ which achieves the lowest KL divergence to the true distribution:
\begin{equation}
    \min \mathcal D[\nu(X); p(X|\theta)] \leq \mathbb{E}_{q(\Theta)}\left[ \mathcal D[\nu(X);p(X|\Theta) \right] = \mathcal R[q] - \mathbb{H}[\nu]
\end{equation}

Unfortunately, the true data-distribution is unknown. Maximum Likelihood and Bayesian Inference differ in how they handle the unknown $\nu(X)$.  Maximum Likelihood 
blazes ahead, replacing the true inferential risk with
the empirical inferential risk:
\begin{equation}
    \overline{\mathcal R}_N[q; x^N] \equiv \mathbb{E}_{q(\Theta)}\left[ \overline L(\theta; x^N) \right] \qquad \overline L(\theta; x^N) \equiv -\frac 1 N \sum_i \log p(x_i|\Theta),
\end{equation}
replacing the expectation with the average over $N$ samples from the true distribution. This creates the 
danger of \emph{overfitting} to the particular sample
of data chosen.  It seeks the parameter setting $\theta$ such that $p(X|\theta)$ is as close as possible to the
\emph{empirical distribution} $\overline \nu(X) = \frac 1 N \sum_i \delta(X - x_i)$ as possible:
\begin{equation}
    \min \mathcal D[\overline \nu(X); p(X|\theta)] \leq \mathbb{E}_{q(\Theta)} \left[ \mathcal D[ \overline \nu(X);  p(X|\Theta) \right] = \overline{\mathcal R}_N[q] - \mathbb{H}[\overline \nu].
\end{equation}
Maximum likelihood closes in on $\overline \nu(X)$ rather than $\nu(X)$.

Bayesian inference on the other hand minimizes what is 
aside from constants with regards to the optimization
a \emph{stochastic upper bound} on the true inferential risk~\citep{knoblauch}.  The Bayesian posterior is the solution to what might be called the \emph{inferential risk}~\citep{pacmbayes}:
\begin{equation}
    \label{eqn:infrisk}
    \widetilde{\mathcal R}_N[q; r, x^N] \equiv \mathbb{E}_{q(\Theta)}\left[ 
    \overline L(\theta; x^N) \right] + \tau \KL\left[q(\Theta); r(\Theta)\right].
\end{equation}
This inferential risk can be motivated as a probably-approximately-correct (PAC) bound on the true risk.  These can be motivated by appealing to the \emph{Compression Lemma}~\citep{banerjee}:
\begin{equation}
    \mathbb{E}_{q(\Theta)}[ \phi(\Theta) ] \leq \tau \log \mathbb{E}_{r(\Theta)}\left[ e^{\phi(\Theta)/\tau} \right] + \tau \KL[q(\Theta);r(\Theta)].
    \label{eqn:compression}
\end{equation}
The compression lemma let's us relate the expected value of a function $\phi(\theta)$ under one distribution $q(\Theta)$ in terms of the log of the expected value of the exponential of that function on another distribution $r(\Theta)$ and the Kullback-Leibler divergence between the two distributions.  Most PAC-Bounds can then be found by choosing as our function $\phi(\theta)$ a difference between a true and empirical loss. For example, if we take:
\begin{equation}
    \phi(\theta) \equiv L(\theta) - \overline L(\theta; x^N) 
\end{equation}
after substituting into~\cref{eqn:compression} we obtain:
\begin{multline}
    \mathbb{E}_{q(\Theta)}[L(\theta)] \leq \mathbb{E}_{q(\Theta)}\left[\overline L(\theta; x^N) \right] + \tau \KL[q(\Theta); r(\Theta)] \\
    + \tau \log \mathbb{E}_{r(\Theta)}\left[e^{\frac 1 \tau(L(\Theta) - \overline L(\Theta; x^N))} \right].
\end{multline}
The first line is~\cref{eqn:infrisk} above, the second line is the 
remaining term from the Compression Lemma (\cref{eqn:compression}). This is a random variable itself due to its dependence on the dataset $(x^N)$, but we can invoke a logarithmic form of Markov's inequality:
\begin{equation}
    \Pr(\log Z \leq \log \mathbb{E}[Z] - \log \xi) \geq 1 - \xi 
\end{equation}
in order to transform the remaining term into a constant, ensuring that with probability at least $1-\xi$:
\begin{multline}
    \label{eqn:pac}
    \mathbb{E}_{q(\Theta)}[L(\theta)] \leq \mathbb{E}_{q(\Theta)}\left[\overline L(\theta; x^N) \right] + \tau \KL[q(\Theta); r(\Theta)] \\
    + \tau \log \mathbb{E}_{r(\Theta)}\mathbb{E}_{\nu(x^N)}\left[e^{\frac 1 \tau (L(\Theta) - \overline L(\Theta; x^N))} \right] - \log \xi.
\end{multline}
In this way, Bayesian inference can be viewed as minimizing an upper bound on the true risk $\mathbb{E}_{q(\Theta)}[L(\Theta)]$, mitigating our concerns about overfitting.  Crucially notice that the terms on the second line are independent of $q(\Theta)$ and so minimizing~\cref{eqn:infrisk} is equivalent to minimizing~\cref{eqn:pac} as far as the parameter distribution $q(\Theta)$ is concerned.
For the same reason, we are not allowed to fig our likelihood $p(x|\theta)$ or our prior $r(\Theta)$ using~\cref{eqn:infrisk} if we wanted to maintain
our bound as they participate in the terms we are dropping. Intuitively, we can assure ourselves that we won't overfit too severely if 
we keep our posterior distribution close to some prior that we specified before we looked at the data.
